A Survey on Deep Learning Event Extraction: Approaches and Applications

Event extraction (EE) is a crucial research task for promptly apprehending event information from massive textual data. With the rapid development of deep learning, EE based on deep learning technology has become a research hotspot. Numerous methods, datasets, and evaluation metrics have been proposed in the literature, raising the need for a comprehensive and updated survey. This article fills the research gap by reviewing the state-of-the-art approaches, especially focusing on the general domain EE based on deep learning models. We introduce a new literature classification of current general domain EE research according to the task definition. Afterward, we summarize the paradigm and models of EE approaches, and then discuss each of them in detail. As an important aspect, we summarize the benchmarks that support tests of predictions and evaluation metrics. A comprehensive comparison among different approaches is also provided in this survey. Finally, we conclude by summarizing future research directions facing the research area.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> del.tex <==


\begin{table*}[t]
\centering
\caption{Basic information based on different models. ED: event detection, AE: argument extraction, NER: named entity recognition, MRC: machine reading comprehension.}
\label{tab:BasicInformation}
% \renewcommand\arraystretch{1.2}
 \linespread{2}
% \resizebox{\textwidth}{!}{
\begin{tabular}{c|cccccccc}
\toprule
\textbf{Year} & \textbf{Model}  & \textbf{Domain}      & \textbf{Venue} & \textbf{Paradigms} & \textbf{Datasets} &\textbf{ED}&\textbf{AE} &\textbf{NER} \\\hline
\multirow{11}{*}{2021} & BRAD \cite{lai2021event} &supervised & ACL/IJCNLP &Pipeline & ACE, BRAD &\checkmark &\checkmark &\checkmark \\
&TEXT2EVENT \cite{lu2021text2event} & supervised & ACL/IJCNLP &Pipeline& ACE05-EN, ERE-EN &\checkmark &\checkmark &\checkmark \\
& CasEE \cite{sheng2021casee} & supervised & ACL/IJCNLP(Findings)&Pipeline & FewFC &\checkmark &\checkmark &\checkmark \\
&CLEVE \cite{wang2021cleve} &supervised & ACL/IJCNLP &Pipeline& ACE, MAVEN &\checkmark &\checkmark &\checkmark \\
&FEAE \cite{wei2021trigger} &supervised & ACL/IJCNLP &Pipeline& RAMS &\checkmark &\checkmark &\checkmark \\
&GIT \cite{xu2021document} &supervised &ACL/IJCNLP &Pipeline& ChFinAnn \footnote{http://www.cninfo.com.cn/new/index} &  \checkmark &\checkmark &\checkmark \\
&NoFPFN \cite{zheng2021revisiting} &supervised &ACL/IJCNLP(Findings)&Pipeline& ChFinAnn &  \checkmark &\checkmark &\checkmark \\

&GATE \cite{DBLP:conf/aaai/AhmadPC21}   &  cross-lingual
 & AAAI  & ACE& \checkmark&\checkmark&\checkmark\\

& DualQA \cite{DBLP:conf/aaai/Zhou0ZWXL21}   &  semi-supervised
 & AAAI  & ACE, FewFC& -&\checkmark&-\\

&GRIT \cite{DBLP:conf/eacl/DuRC21}&supervised&EACL&MUC-4& \checkmark&\checkmark&-\\

& Wen et al.\cite{DBLP:conf/naacl/WenQJNHSTR21}  &supervised &NAACL-HLT&ACE& \checkmark&\checkmark&-\\\cline{1-8}

\multirow{7}{*}{2020} &SciBERT \cite{DBLP:conf/acl-louhi/WangWL20} &MRC&LOUHI@EMNLP& BioNLP13, GENIA & \checkmark&\checkmark&-\\

& HPNet \cite{DBLP:conf/coling/HuangZTTX20} &supervised& COLING& ACE2005, TAC2015 & \checkmark&\checkmark&-\\

 & M2E2 \cite{DBLP:conf/acl/LiZZWLJC20} & weakly supervised&ACL&  M2E2 & \checkmark&\checkmark&-\\

% 2020 & DMB-PN \cite{DBLP:conf/wsdm/DengZKZZC20}        & few-shot & WSDM  & FewEvent& \checkmark&-&-\\\cline{2-8}

 & MQAEE \cite{DBLP:conf/emnlp/LiPCWPLZ20}       & MRC & EMNLP  & ACE& \checkmark&\checkmark&-\\

 & Du et al. \cite{DBLP:conf/emnlp/DuC20}        & MRC & EMNLP  & ACE& \checkmark&\checkmark&-\\

% 2020 & Lai et al. \cite{DBLP:conf/pakdd/LaiDN20}  & few-shot & PAKDD  & ACE, TAC-KBP  &\checkmark&-&- \\\cline{2-8}

 &  Min et al. \cite{DBLP:conf/lrec/MinCZ20}          & few-shot  & LREC  &ACE   &-&\checkmark&-\\

&Chen et al. \cite{DBLP:journals/corr/abs-1912-01586} &supervised&SPNLP@EMNLP&ACE&-&\checkmark&-\\\cline{1-8}

\multirow{18}{*}{2019} & Doc2EDAG \cite{DBLP:conf/emnlp/ZhengCXB19}   & chinese  & EMNLP  &  ChFinAnn  &\checkmark&\checkmark&\checkmark\\

 & Ananya et al \cite{DBLP:conf/emnlp/SubburathinamLJ19} & cross-lingual & EMNLP  &ACE &\checkmark&\checkmark&\checkmark\\
%  \cline{2-8}


 & Chau et al.\cite{DBLP:journals/corr/abs-1912-11334} & open domain & arXiv  & NYT  &\checkmark&\checkmark&- \\

 & Chen et al.\cite{chen2019reading} & MRC & arXiv  & ACE &\checkmark&\checkmark&- \\

 & GAIL-ELMo \cite{DBLP:journals/dint/ZhangJS19} & supervised  & Data Intell.  & ACE &\checkmark&\checkmark&\checkmark \\

 & ODEE-FER \cite{DBLP:conf/acl/LiuHZ19}    & open domain& ACL  & GNBusiness  &\checkmark&\checkmark&\checkmark\\

 & DYGIE++ \cite{DBLP:conf/emnlp/WaddenWLH19} & supervised & EMNLP  & ACE, SciERC, etc.  &\checkmark&\checkmark&\checkmark\\

 & HMEAE \cite{DBLP:conf/emnlp/WangWHLLLSZR19} &supervised  & EMNLP  & ACE, TAC-KBP &-&\checkmark&\checkmark\\

 & Han et al. \cite{DBLP:conf/emnlp/HanNP19} & supervised & EMNLP  & TB-Dense, MATRES &\checkmark&\checkmark&\checkmark\\

% 2019 & \cite{DBLP:conf/emnlp/SubburathinamLJ19} & multilingual & EMNLP  & & \\\cline{2-8}

 & PLMEE \cite{DBLP:conf/acl/YangFQKL19}          & data generation & ACL& ACE &\checkmark&\checkmark&\checkmark\\

 & AEM \cite{DBLP:conf/emnlp/WangZH19}          & open domain & EMNLP & FSD, Twitter, et al. &\checkmark&\checkmark&\checkmark \\

 & JointTransition \cite{DBLP:conf/ijcai/ZhangQZLJ19}          & supervised & IJCAI & ACE &\checkmark&\checkmark&\checkmark \\

 & Li et al. \cite{DBLP:conf/naacl/LiHJ019}          & external knowledge & NAACL & Genia 2011 &\checkmark&\checkmark&\checkmark \\

 & MLM-Joint \cite{DBLP:journals/access/LiCHWJ19}          & unsupervised & IEEE Access & DUC 2004, ACE &\checkmark&\checkmark&\checkmark \\

 & Joint3EE \cite{DBLP:conf/aaai/NguyenN19}          &supervised  & AAAI & ACE &\checkmark&\checkmark&\checkmark \\

 & Chan et al. \cite{DBLP:conf/acl/ChanFQM19} & supervised & ACL  & ACE &\checkmark&\checkmark&\checkmark \\

%  2019 & Davani et al. \cite{DBLP:conf/emnlp/DavaniYAKPGDBMR19} & data generation & EMNLP  &  FBI
% dataset & \\\cline{2-8}

 & Davani et al. \cite{DBLP:conf/emnlp/DavaniYAKPGDBMR19} & open domain & EMNLP  &FBI dataset   &\checkmark&\checkmark&-\\

% 2019 & Liu et al. \cite{DBLP:conf/emnlp/LiuCLZ19}          & cross-lingual & EMNLP  & ACE, TAC-KBP  &\checkmark&-&-  \\\cline{2-8}

 & Li et al. \cite{DBLP:conf/acl/LiYSLYCZL19}         & MRC & ACL    & ACE, CoNLL04   &\checkmark&\checkmark&-\\\cline{1-8}

% 2019 & JOINT3EE         &  &     &  &\\\cline{2-8}


\multirow{9}{*}{2018}  & DCFEE~ \cite{DBLP:conf/acl/YangCLXZ18} & chinese   & ACL &NO.(ANN, POS, NEG)& \checkmark &\checkmark &-\\

% 2018 & Ferguson et al. \cite{DBLP:conf/naacl/FergusonLWH18}     & semi-supervised & NAACL  & ACE, TAC-KBP &\checkmark&\checkmark&\checkmark  \\\cline{2-8}

 & Zeng et al. \cite{DBLP:conf/aaai/ZengFMWYSZ18}     & data generation & AAAI  & FBWiki, ACE &\checkmark&\checkmark&- \\

 & Huang et al.\cite{DBLP:conf/acl/DaganJVHCR18} & zero-shot & ACL &ACE &\checkmark&\checkmark&-  \\

 & DEEB-RNN \cite{DBLP:conf/acl/ZhaoJWC18} & supervised & ACL &ACE &\checkmark&-&-  \\

 & SELF \cite{DBLP:conf/acl/ZhouZHZ18} & supervised & ACL &ACE, TAC-KBP &\checkmark&-&-  \\


 & DBRNN \cite{DBLP:conf/aaai/ShaQCS18}          & supervised & AAAI &ACE &\checkmark&\checkmark&\checkmark \\

 & GMLATT \cite{DBLP:conf/aaai/Liu00018}        & cross lingual & AAAI &ACE &\checkmark&-&- \\

 & JMEE \cite{DBLP:conf/emnlp/LiuLH18}          & supervised & EMNLP & ACE &\checkmark&\checkmark&\checkmark \\

 & Ferguson et al.\cite{DBLP:conf/naacl/FergusonLWH18}          & semi-supervised & NAACL&ACE, TAC-KBP &\checkmark&\checkmark&- \\\cline{1-8}

\multirow{2}{*}{2017} & DMCNN-MIL \cite{DBLP:conf/acl/ChenLZLZ17}          & data generation  & ACL& ACE &\checkmark&\checkmark&-  \\

%  2017 & Levy et al. \cite{DBLP:conf/conll/LevySCZ17}         & MRC & CoNLL  & - & \\\cline{2-8}

 & Liu et al.\cite{DBLP:conf/acl/LiuCLZ17} & supervised & ACL &ACE &\checkmark&-&-  \\\cline{1-8}

\multirow{8}{*}{2016}  & RBPB~ \cite{DBLP:conf/acl/ShaLLLCS16}  & supervised & ACL  & ACE &\checkmark&\checkmark&- \\

 & Zeng et al.\cite{DBLP:conf/nlpcc/ZengYFWZ16}        & chinese  & NLPCC  &  ACE  &\checkmark&\checkmark&- \\

% 2016 & HNN \cite{DBLP:conf/acl/FengHTJQL16} & -  & ACL  &  ACE  &\checkmark&-&- \\\cline{2-8}

 & JRNN \cite{DBLP:conf/naacl/NguyenCG16} & supervised & NAACL  & ACE &\checkmark&\checkmark&\checkmark \\

 & JOINTEVENTENTITY \cite{DBLP:conf/naacl/YangM16} & supervised & NAACL  & ACE &\checkmark&\checkmark&\checkmark \\

 & BDLSTM-TNNs \cite{DBLP:conf/cncl/ChenLHL016}  &  supervised& CCL  & ACE &\checkmark&\checkmark&\checkmark \\

 & Huang et al. \cite{DBLP:conf/acl/HuangCFJVHS16}  &supervised  & ACL  & ERE, ACE &\checkmark&\checkmark&- \\

 & Liu et al. \cite{DBLP:conf/acl/LiuCHL016}  &supervised  & ACL  & ACE &\checkmark&-&- \\

 & Hsi et al.\cite{DBLP:conf/coling/HsiYCX16}         & multilingual & COLING & ACE &\checkmark&\checkmark&\checkmark\\\cline{1-8}

\multirow{1}{*}{2015}  & DMCNN~ \cite{DBLP:conf/acl/ChenXLZ015}  &supervised  & ACL & ACE&\checkmark&\checkmark&-  \\
\bottomrule
\end{tabular}
% }
\end{table*}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/flowchart.pdf}
%     \caption{The architecture of this paper. The event extraction is introduced from basic information, extraction paradigm, extraction model and extraction corpus aspects. }
%     \label{figure1}
%     \label{img}
% \end{figure} 






% \smartdiagram[circular diagram:clockwise]{Basic, Paradigm, Model, Datasets and Metrics, Results, Future Trends}




\begin{table*}[t]
\centering
\caption{Basic information based on different models. ED: event detection, AE: argument extraction, NER: named entity recognition, MRC: machine reading comprehension.}
\label{tab:BasicInformation}
% \renewcommand\arraystretch{1.2}
 \linespread{2}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccccccc}
\toprule
\textbf{Year} & \textbf{Model}  & \textbf{Supervise}   & \textbf{Task}     & \textbf{Paradigms} & \textbf{Datasets} &\textbf{ED}&\textbf{AE} &\textbf{NER} \\\hline
\multirow{11}{*}{2021} & BRAD \cite{lai2021event} &Supervised   & Sequence Labeling & Joint & ACE, BRAD  &\checkmark &\checkmark& \checkmark\\
&TEXT2EVENT \cite{lu2021text2event} & supervised &Generation & Joint& ACE05-EN, ERE-EN &\checkmark &\checkmark &\checkmark \\
& CasEE \cite{sheng2021casee} & supervised&Sequence Labeling & Joint & FewFC &\checkmark &\checkmark &\checkmark \\
&CLEVE \cite{wang2021cleve} &supervised &Classification& Pipeline& ACE, MAVEN &\checkmark &\checkmark &\checkmark \\
&FEAE \cite{wei2021trigger} &supervised &Classification& Pipeline& RAMS &\checkmark &\checkmark &\checkmark \\
&GIT \cite{xu2021document} &supervised &Classification &Pipeline& ChFinAnn \footnote{http://www.cninfo.com.cn/new/index} &  \checkmark &\checkmark &\checkmark \\
&NoFPFN \cite{zheng2021revisiting} &supervised &Classification&Pipeline& ChFinAnn &  \checkmark &\checkmark &\checkmark \\

&GATE \cite{DBLP:conf/aaai/AhmadPC21}   &  cross-lingual&Classification
 & Pipeline  & ACE& \checkmark&\checkmark&\checkmark\\

& DualQA \cite{DBLP:conf/aaai/Zhou0ZWXL21}   &  semi-supervised&Classification
 & Pipeline  & ACE, FewFC& -&\checkmark&-\\

&GRIT \cite{DBLP:conf/eacl/DuRC21}&supervised&Classification&Pipeline&MUC-4& \checkmark&\checkmark&-\\

& Wen et al.\cite{DBLP:conf/naacl/WenQJNHSTR21}  &supervised&Classification &Pipeline&ACE& \checkmark&\checkmark&-\\\cline{1-9}

\multirow{7}{*}{2020} &SciBERT \cite{DBLP:conf/acl-louhi/WangWL20} &MRC  &Classification  &Pipeline& BioNLP13, GENIA & \checkmark&\checkmark&-\\

& HPNet \cite{DBLP:conf/coling/HuangZTTX20} &supervised  & Classification  & Pipeline& ACE2005, TAC2015 & \checkmark&\checkmark&-\\

 & M2E2 \cite{DBLP:conf/acl/LiZZWLJC20} & weakly supervised &Classification &Pipeline&  M2E2 & \checkmark&\checkmark&-\\

% 2020 & DMB-PN \cite{DBLP:conf/wsdm/DengZKZZC20}        & few-shot & WSDM  & FewEvent& \checkmark&-&-\\\cline{2-8}

 & MQAEE \cite{DBLP:conf/emnlp/LiPCWPLZ20}       & MRC&Classification & Pipeline  & ACE& \checkmark&\checkmark&-\\

 & Du et al. \cite{DBLP:conf/emnlp/DuC20}        & MRC&Classification & Pipeline  & ACE& \checkmark&\checkmark&-\\

% 2020 & Lai et al. \cite{DBLP:conf/pakdd/LaiDN20}  & few-shot & PAKDD  & ACE, TAC-KBP  &\checkmark&-&- \\\cline{2-8}

 &  Min et al. \cite{DBLP:conf/lrec/MinCZ20}          & few-shot  &Classification& Pipeline  &ACE   &-&\checkmark&-\\

&Chen et al. \cite{DBLP:journals/corr/abs-1912-01586} &supervised&Classification&Pipeline&ACE&-&\checkmark&-\\\cline{1-9}

\multirow{18}{*}{2019} & Doc2EDAG \cite{DBLP:conf/emnlp/ZhengCXB19}   & chinese &Classification & Pipeline  &  ChFinAnn  &\checkmark&\checkmark&\checkmark\\

 & Ananya et al \cite{DBLP:conf/emnlp/SubburathinamLJ19} & cross-lingual&Classification & Pipeline  &ACE &\checkmark&\checkmark&\checkmark\\
%  \cline{2-8}


 & Chau et al.\cite{DBLP:journals/corr/abs-1912-11334} & open domain &Classification& Pipeline  & NYT  &\checkmark&\checkmark&- \\

 & Chen et al.\cite{chen2019reading} & MRC&Classification & Pipeline  & ACE &\checkmark&\checkmark&- \\

 & GAIL-ELMo \cite{DBLP:journals/dint/ZhangJS19} & supervised&Classification & Pipeline  & ACE &\checkmark&\checkmark&\checkmark \\

 & ODEE-FER \cite{DBLP:conf/acl/LiuHZ19}    & open domain&Classification& Pipeline  & GNBusiness  &\checkmark&\checkmark&\checkmark\\

 & DYGIE++ \cite{DBLP:conf/emnlp/WaddenWLH19} & supervised&Classification & Pipeline  & ACE, SciERC, etc.  &\checkmark&\checkmark&\checkmark\\

 & HMEAE \cite{DBLP:conf/emnlp/WangWHLLLSZR19} &supervised &Classification & Pipeline  & ACE, TAC-KBP &-&\checkmark&\checkmark\\

 & Han et al. \cite{DBLP:conf/emnlp/HanNP19} & supervised &Classification& Pipeline  & TB-Dense, MATRES &\checkmark&\checkmark&\checkmark\\

% 2019 & \cite{DBLP:conf/emnlp/SubburathinamLJ19} & multilingual & EMNLP  & & \\\cline{2-8}

 & PLMEE \cite{DBLP:conf/acl/YangFQKL19}          & data generation &Classification& Pipeline& ACE &\checkmark&\checkmark&\checkmark\\

 & AEM \cite{DBLP:conf/emnlp/WangZH19}          & open domain &Classification& Pipeline & FSD, Twitter, et al. &\checkmark&\checkmark&\checkmark \\

 & JointTransition \cite{DBLP:conf/ijcai/ZhangQZLJ19}          & supervised&Classification & Pipeline & ACE &\checkmark&\checkmark&\checkmark \\

 & Li et al. \cite{DBLP:conf/naacl/LiHJ019}          & external knowledge&Classification & Pipeline & Genia 2011 &\checkmark&\checkmark&\checkmark \\

 & MLM-Joint \cite{DBLP:journals/access/LiCHWJ19}          & unsupervised&Classification & Pipeline & DUC 2004, ACE &\checkmark&\checkmark&\checkmark \\

 & Joint3EE \cite{DBLP:conf/aaai/NguyenN19}          &supervised &Classification & Pipeline & ACE &\checkmark&\checkmark&\checkmark \\

 & Chan et al. \cite{DBLP:conf/acl/ChanFQM19} & supervised &Classification& Pipeline  & ACE &\checkmark&\checkmark&\checkmark \\

%  2019 & Davani et al. \cite{DBLP:conf/emnlp/DavaniYAKPGDBMR19} & data generation & EMNLP  &  FBI
% dataset & \\\cline{2-8}

 & Davani et al. \cite{DBLP:conf/emnlp/DavaniYAKPGDBMR19} & open domain &Classification& Pipeline  &FBI dataset   &\checkmark&\checkmark&-\\

% 2019 & Liu et al. \cite{DBLP:conf/emnlp/LiuCLZ19}          & cross-lingual & EMNLP  & ACE, TAC-KBP  &\checkmark&-&-  \\\cline{2-8}

 & Li et al. \cite{DBLP:conf/acl/LiYSLYCZL19}         & MRC&Classification & Pipeline    & ACE, CoNLL04   &\checkmark&\checkmark&-\\\cline{1-9}

% 2019 & JOINT3EE         &  &     &  &\\\cline{2-8}


\multirow{9}{*}{2018}  & DCFEE~ \cite{DBLP:conf/acl/YangCLXZ18} & chinese  &Classification & Pipeline &NO.(ANN, POS, NEG)& \checkmark &\checkmark &-\\

% 2018 & Ferguson et al. \cite{DBLP:conf/naacl/FergusonLWH18}     & semi-supervised & NAACL  & ACE, TAC-KBP &\checkmark&\checkmark&\checkmark  \\\cline{2-8}

 & Zeng et al. \cite{DBLP:conf/aaai/ZengFMWYSZ18}     & data generation&Classification & Pipeline  & FBWiki, ACE &\checkmark&\checkmark&- \\

 & Huang et al.\cite{DBLP:conf/acl/DaganJVHCR18} & zero-shot&Classification & Pipeline &ACE &\checkmark&\checkmark&-  \\

 & DEEB-RNN \cite{DBLP:conf/acl/ZhaoJWC18} & supervised&Classification & Pipeline &ACE &\checkmark&-&-  \\

 & SELF \cite{DBLP:conf/acl/ZhouZHZ18} & supervised&Classification & Pipeline &ACE, TAC-KBP &\checkmark&-&-  \\


 & DBRNN \cite{DBLP:conf/aaai/ShaQCS18}          & supervised&Classification & Pipeline &ACE &\checkmark&\checkmark&\checkmark \\

 & GMLATT \cite{DBLP:conf/aaai/Liu00018}        & cross lingual&Classification & Pipeline &ACE &\checkmark&-&- \\

 & JMEE \cite{DBLP:conf/emnlp/LiuLH18}          & supervised &Classification& Pipeline & ACE &\checkmark&\checkmark&\checkmark \\

 & Ferguson et al.\cite{DBLP:conf/naacl/FergusonLWH18}          & semi-supervised &Classification& Pipeline&ACE, TAC-KBP &\checkmark&\checkmark&- \\\cline{1-9}

\multirow{2}{*}{2017} & DMCNN-MIL \cite{DBLP:conf/acl/ChenLZLZ17}          & data generation &Classification & Pipeline& ACE &\checkmark&\checkmark&-  \\

%  2017 & Levy et al. \cite{DBLP:conf/conll/LevySCZ17}         & MRC & CoNLL  & - & \\\cline{2-8}

 & Liu et al.\cite{DBLP:conf/acl/LiuCLZ17} & supervised&Classification & Pipeline &ACE &\checkmark&-&-  \\\cline{1-9}

\multirow{8}{*}{2016}  & RBPB~ \cite{DBLP:conf/acl/ShaLLLCS16}  & supervised &Classification& Pipeline  & ACE &\checkmark&\checkmark&- \\

 & Zeng et al.\cite{DBLP:conf/nlpcc/ZengYFWZ16}        & chinese &Classification & Pipeline  &  ACE  &\checkmark&\checkmark&- \\

% 2016 & HNN \cite{DBLP:conf/acl/FengHTJQL16} & -  & ACL  &  ACE  &\checkmark&-&- \\\cline{2-8}

 & JRNN \cite{DBLP:conf/naacl/NguyenCG16} & supervised&Classification & Pipeline  & ACE &\checkmark&\checkmark&\checkmark \\

 & JOINTEVENTENTITY \cite{DBLP:conf/naacl/YangM16} & supervised&Classification & Pipeline  & ACE &\checkmark&\checkmark&\checkmark \\

 & BDLSTM-TNNs \cite{DBLP:conf/cncl/ChenLHL016}  &  supervised&Classification& Pipeline  & ACE &\checkmark&\checkmark&\checkmark \\

 & Huang et al. \cite{DBLP:conf/acl/HuangCFJVHS16}  &supervised  &Classification& Pipeline  & ERE, ACE &\checkmark&\checkmark&- \\

 & Liu et al. \cite{DBLP:conf/acl/LiuCHL016}  &supervised  &Classification& Pipeline  & ACE &\checkmark&-&- \\

 & Hsi et al.\cite{DBLP:conf/coling/HsiYCX16}         & multilingual&Classification & Pipeline & ACE &\checkmark&\checkmark&\checkmark\\\cline{1-9}

\multirow{1}{*}{2015}  & DMCNN~ \cite{DBLP:conf/acl/ChenXLZ015}  &supervised &Classification & Pipeline & ACE&\checkmark&\checkmark&-  \\
\bottomrule
\end{tabular}
}
\end{table*}




\begin{table*}[t]
\centering
\caption{Comparison of event extraction methods on ACE 2005. We show the performance of trigger classification and argument role classification sub-tasks.}
\label{ace}
\resizebox{\textwidth}{!}{
% \scalebox{0.98}{
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Year-Method}}& \multirow{2}{*}{\textbf{Neural Network}} & \multirow{2}{*}{\textbf{External Resource}} &\multirow{2}{*}{\textbf{Paradigm}}  & \multicolumn{3}{c}{\textbf{Trigger Classification}}       & \multicolumn{3}{c}{\textbf{Role Classification}}             \\\cline{5-10}
  & &  &  & \textbf{P}     &\textbf{R}      & \textbf{F1}   & \textbf{P}       & \textbf{R}      & \textbf{F1}   \\\hline 
2008 - Ji et al. \cite{DBLP:conf/acl/JiG08}      & -     & -  &-  & 60.2 & 76.4 & 67.3     & 51.3    & 36.4     & 42.6    \\\hline  
2010 - Liao et al. \cite{DBLP:conf/acl/LiaoG10} & -  & - &-  & 68.7  & 68.9   & 68.8    & 45.1  & 44.1  & 44.6   \\\hline 
2011 - Hong et al. \cite{DBLP:conf/acl/HongZMYZZ11}    & -  & - &-  & 72.9  & 64.3     & 68.3   & 51.6   & 45.5     & 48.4    \\\hline 
2013 - Li et al. \cite{DBLP:conf/acl/LiJH13} & - & -  &-& 73.7 & 62.3 & 67.5 & 64.7 & 44.4 & 52.7   \\\hline 
2015 - Nguyen et al. \cite{DBLP:conf/acl/NguyenG15}  & \checkmark  & - &- & 71.8  & 66.4  & 69.0  & -    & -   & -     \\\hline 
2015 - DMCNN \cite{DBLP:conf/acl/ChenXLZ015}   & \checkmark & - &Pipeline & 75.6       & 63.6  & 69.1     & 62.2  & 46.9    & 53.5     \\\hline 
2016 - JRNN \cite{DBLP:conf/naacl/NguyenCG16} & \checkmark   & - &Joint & 66.0  & 73.0   & 69.3   & 54.2   & \textbf{56.7}   & 55.4  \\\hline 
2016 - JOINTEVENTENTIT \cite{DBLP:conf/naacl/YangM16}  & -  & - &Joint  & 75.1  & 63.3  & 68.7  & \textbf{70.6}   & 36.9   & 48.4   \\\hline 
2016 - Liu et al. \cite{DBLP:conf/acl/LiuCHL016}  & \checkmark  & \checkmark &Joint & 77.6   & 65.2  & 70.7 & - & -   & -  \\\hline 
2016 - NC-CNN \cite{DBLP:conf/emnlp/NguyenG16}  & \checkmark   & - &- & -  & -  & 71.3 & -  & -  & -  \\\hline 
2016 - HNN \cite{DBLP:conf/acl/FengHTJQL16} & \checkmark  & - &- & 84.6  & 64.9  & 73.4  & -  & -   & -    \\\hline 

2016 - Huang et al.\cite{DBLP:conf/acl/HuangCFJVHS16}& \checkmark  & \checkmark &Joint  & 80.7  & 50.1  & 61.8  & 51.9  & 39.4   & 44.8     \\\hline

2016 - BDLSTM-TNNs \cite{DBLP:conf/cncl/ChenLHL016}&  \checkmark  &  - & Joint &  75.3 & 63.4 & 68.9  & 62.9  & 47.5   & 54.1    \\\hline

2016 - Zeng et al. \cite{DBLP:conf/nlpcc/ZengYFWZ16}& \checkmark  & - & Joint& 69.8  & 59.9 & 64.5  & 47.3  &46.6    &  46.9   \\\hline

2016 - RBPB \cite{DBLP:conf/acl/ShaLLLCS16}& \checkmark  & - &Pipeline & 70.3  & 67.5 & 68.9  & 54.1  &  53.5  &  53.8   \\\hline

2017 - Liu et al. \cite{DBLP:conf/acl/LiuCLZ17} & \checkmark  & - &Pipeline& 78.0 & 66.3  & 71.7 & -  & -  & -   \\\hline 
2017 - DMCNN-MIL \cite{DBLP:conf/acl/ChenLZLZ17}  & \checkmark  & \checkmark  &Joint   & 75.5  & 66.0    & 70.5  & 62.8  & 50.1 & 55.7       \\\hline        

2018 - DEEB-RNN \cite{DBLP:conf/acl/ZhaoJWC18}  & \checkmark  & - &Pipeline & 72.3  & 75.8 & 74  & -  & -   & -    \\\hline

2018 - SELF \cite{DBLP:conf/acl/ZhouZHZ18}  & \checkmark   & - &Pipeline & 71.3  & 74.7 & 73.0  & -  &-    &   -  \\\hline

2018 - DBRNN \cite{DBLP:conf/aaai/ShaQCS18}  & \checkmark   &  - &Joint&  74.1 & 69.8 & 71.9  & 66.2  & 52.8   &  58.7   \\\hline

2018 - GMLATT \cite{DBLP:conf/aaai/Liu00018} &  \checkmark & - &Joint  & 78.9  & 66.9 & 72.4  &  - &  -  & -    \\\hline

2018 - JMEE\cite{DBLP:conf/emnlp/LiuLH18} & \checkmark  & - &Joint & 76.3  & 71.3 & 73.7   &  66.8 &  54.9  & 60.3    \\\hline

2018 - Zeng et al. \cite{DBLP:conf/aaai/ZengFMWYSZ18}      & \checkmark  &\checkmark & Pipeline & \textbf{85.3}  & 79.9 & \textbf{82.5}  & 41.9  & 34.6   &  37.9   \\\hline

2019 - Joint3EE \cite{DBLP:conf/aaai/NguyenN19}     &  \checkmark &  - & Joint&  68.0 & 71.8 &  69.8 & 52.1  &  52.1  & 52.1    \\\hline

2019 - Liu et al.\cite{DBLP:conf/emnlp/LiuCLZ19}       & \checkmark  &  -& Joint & 62.5  & 35.7 &  45.4 & -  &  -  & -    \\\hline

2019 - Chen et al.\cite{chen2019reading} &  \checkmark  &  - & Joint & 66.7  & 74.7 & 70.5  & 44.3  &  40.7  &  42.4   \\\hline

2019 - GAIL-ELMo \cite{DBLP:journals/dint/ZhangJS19} &   \checkmark &  - & Joint & 74.8  & 69.4 & 72.0  & 61.6  &  45.7  &  52.4   \\\hline

2019 - DYGIE++ \cite{DBLP:conf/emnlp/WaddenWLH19} & \checkmark  & - & Joint  & -  & - & 69.7  &  - &  -  & 48.8    \\\hline

2019 - HMEAE \cite{DBLP:conf/emnlp/WangWHLLLSZR19} &  \checkmark  &  -& Joint &  - & - &  - &  62.2 &  56.6  & 59.3    \\\hline

2019 - JointTransition \cite{DBLP:conf/ijcai/ZhangQZLJ19}     & \checkmark  & - & Joint  &  74.4 & 73.2 & 73.8  & 55.7  & 51.1   &  53.3   \\\hline

2019 - PLMEE \cite{DBLP:conf/acl/YangFQKL19}  &  \checkmark &  - & Joint & 81.0  & \textbf{80.4} & 80.7  & 62.3  &  54.2  & 58.0    \\\hline

2020 - Chen et al. \cite{DBLP:conf/acl-spnlp/ChenCEWD20}  &  \checkmark &  -& Pipeline & 66.7  & 74.7 & 70.5  & 44.3  &  40.7  & 42.4    \\\hline
2020 - MQAEE \cite{DBLP:conf/emnlp/LiPCWPLZ20}  &  \checkmark &  -& Pipeline & -  & - & 73.8  & -  &  - & 55.0    \\\hline

2020 - Du et al. \cite{DBLP:conf/emnlp/DuC20}  &  \checkmark &  - &Pipeline & 71.1  & 73.7 & 72.3  & 56.7  &  50.2  & 53.3    \\\hline
2021-Li et al. \cite{DBLP:conf/naacl/LiJH21}   &  \checkmark  &  -& - & -  & - &71.1   & -  &  - &53.7   \\\hline
2021-GATE (En2ZH) \cite{DBLP:conf/aaai/AhmadPC21}   & \checkmark  &  -& Joint & -  & - & -  & -  &  - & \textbf{63.2}  \\\hline
2021-Text2Event \cite{DBLP:journals/corr/abs-2106-09232}  &  \checkmark &  -& Joint & 69.6  &74.4 & 71.9  & 52.5 &  55.2 & 53.8    \\
\bottomrule
\end{tabular}
}
\end{table*}


